Efficient Deep Image Denoising via Class Specific Convolution

Deep neural networks have been widely used in image denoising during the past few years. Even though they achieve great success on this problem, they are computationally inefficient which makes them inappropriate to be implemented in mobile devices. In this paper, we propose an efficient deep neural network for image denoising based on pixel-wise classification. Despite using a computationally efficient network cannot effectively remove the noises from any content, it is still capable to denoise from a specific type of pattern or texture. The proposed method follows such a divide and conquer scheme. We first use an efficient U-net to pixel-wisely classify pixels in the noisy image based on the local gradient statistics. Then we replace part of the convolution layers in existing denoising networks by the proposed Class Specific Convolution layers (CSConv) which use different weights for different classes of pixels. Quantitative and qualitative evaluations on public datasets demonstrate that the proposed method can reduce the computational costs without sacrificing the performance compared to state-of-the-art algorithms.

==> tables.tex <==
(click "Generate" to refresh) Copy to clipboard
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\begin{table}[]
\begin{tabular}{lllllllllllll}
Dataset                   & Noise Level                & DnCNN & CARN  & EDSR  & FC-AIDE & RED   & MemNet & FOCNet & SGN   & KPN   & SC-CARN & SC-EDSR \\
\multirow{3}{*}{BSD68}    & \textbackslash{}sigma = 15 & -     & 32.10 & 32.16 & 31.78   & -     & -      & 31.83  & -     & -     & 32.01   & 32.08   \\
                          & \textbackslash{}sigma = 25 & 29.58 & 29.63 & 29.70 & 29.31   & 29.66 & 29.39  & 29.38  & -     & 29.55 & 29.65   & 29.76   \\
                          & \textbackslash{}sigma = 50 & 26.54 & 26,70 & 26,84 & 26.38   & 26.67 & 26.69  & 26.50  & 26.43 & -     & 27.21   & 27.31   \\
\multirow{3}{*}{Urban100} & \textbackslash{}sigma=15   & -     & 32.95 & 33.10 & 32.65   & -     & -      & 33.15  & -     & -     & 32.76   & 32.93   \\
                          & \textbackslash{}sigma=25   & -     & 30.02 & 30.36 & 30.05   & 29.93 & 29.69  & 30.64  & -     & 29.72 & 30.17   & 29.83   \\
                          & \textbackslash{}sigma=50   & -     & 26.33 & 26,85 & 26.42   & -     & -      & 27.40  &       & -     & 26.76   & 27.07   \\
\multirow{3}{*}{DIV2K}    & \textbackslash{}sigma=15   & -     & 34.04 & 34.14 & -       & -     & -      & -      & -     & -     & 33.94   & 34.03   \\
                          & \textbackslash{}sigma=25   & 31.39 & 31.53 & 31.66 & -       & 31.56 & 31.47  & -      & -     & 31.51 & 31.58   & 31.75   \\
                          & \textbackslash{}sigma=50   & 28.25 & 28.40 & 28.65 & -       & -     & -      & -      & 28.53 & -     & 29.02   & 29.17   \\
\multirow{3}{*}{Set12}    & \textbackslash{}sigma=15   & -     & 33.16 & 33.34 & 32.91   & -     & -      & 33.07  & -     & -     & 33.14   & 33.18   \\
                          & \textbackslash{}sigma=25   & -     & 30.76 & 30.95 & 30.57   & 30.76 & 30.45  & 30.73  & -     & 30.68 & 30.78   & 30.97   \\
                          & \textbackslash{}sigma=50   & -     & 27,58 & 27,86 & 27.42   & 27.50 & 27.48  & 27.68  & -     & -     & 28.16   & 28.33  
\end{tabular}
\end{table}


\begin{table}[]
\begin{tabular}{lllllllllllll}
Dataset  & CS-EDSR & EDSR-16 & EDSR-GT & EDSR-NOISE & EDSR4 & EDSR-CE & CS-CARN & CARN-16 & CARN-GT & CARN-NOISE & CARN4 & CARN-CE \\
BSD68    & 29.76   & 29.60   & 30.224  & 29.42      & 29.69 & 29.69   & 29.65   & 29.36   & 29.9    & 29.36      & 29.62 & 29.51   \\
Urban100 & 30.17   & 29.96   & 30.47   & 29.36      & 30.03 & 30.09   & 29.83   & 29.27   & 29.97   & 29.36      & 29.63 & 29.58   \\
DIV2K    & 31.74   & 31.52   & 32.22   & 31.28      & 31.67 & 31.61   & 31.58   & 31.163  & 31.87   & 31.22      & 31.46 & 31.41   \\
Set12    & 30.97   & 30.78   & 31.39   & 30.40      & 30.85 & 30.88   & 30.78   & 30.40   & 31.00   & 30.31      & 30.65 & 30.59  
\end{tabular}
\end{table}



\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR/SSIM) by EDSR models with feature channels $C_f = 16$ and different number of blocks.}
\label{table:ablationclass}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll} \hline \hline
%Dataset  & CS & 16 & G & N & $\phi_4$ & CE & CS & 16 & G & N & $\phi_4$ & CE \\ \hline
$N_B$    & 16 & 16  & 12   & 12  & 8 & 8   \\
CSConv    & Y & N   & Y   & N  & Y & N   \\
BSD68    & 29.76   & 29.60   & 30.224  & 29.42      & 29.69 & 29.69     \\
Urban100 & 30.17   & 29.96   & 30.47   & 29.36      & 30.03 & 30.09     \\
DIV2K    & 31.74   & 31.52   & 32.22   & 31.28      & 31.67 & 31.61    \\
Set12    & 30.97   & 30.78   & 31.39   & 30.40      & 30.85 & 30.88    \\ \hline\hline
\end{tabular}}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR/SSIM) by different methods.}
\label{table:ablationclass}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll|llllll} \hline \hline
& \multicolumn{6}{c|}{EDSR}  & \multicolumn{6}{c}{CARN} \\
Dataset  & CS & 16 & G & N & $\phi_4$ & CE & CS & 16 & G & N & $\phi_4$ & CE \\ \hline
BSD68    & 29.76   & 29.60   & 30.224  & 29.42      & 29.69 & 29.69   & 29.65   & 29.36   & 29.9    & 29.36      & 29.62 & 29.51   \\
Urban100 & 30.17   & 29.96   & 30.47   & 29.36      & 30.03 & 30.09   & 29.83   & 29.27   & 29.97   & 29.36      & 29.63 & 29.58   \\
DIV2K    & 31.74   & 31.52   & 32.22   & 31.28      & 31.67 & 31.61   & 31.58   & 31.163  & 31.87   & 31.22      & 31.46 & 31.41   \\
Set12    & 30.97   & 30.78   & 31.39   & 30.40      & 30.85 & 30.88   & 30.78   & 30.40   & 31.00   & 30.31      & 30.65 & 30.59  \\ \hline\hline
\end{tabular}}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR/SSIM) by different methods.}
\label{table:ablationclass}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll|llllll} \hline \hline
& \multicolumn{6}{c|}{EDSR}  & \multicolumn{6}{c}{CARN} \\
Dataset  & CS & 16 & G & N & $\phi_4$ & CE & CS & 16 & G & N & $\phi_4$ & CE \\ \hline
BSD68    & 29.76   & 29.60   & 30.224  & 29.42      & 29.69 & 29.69   & 29.65   & 29.36   & 29.9    & 29.36      & 29.62 & 29.51   \\
Urban100 & 30.17   & 29.96   & 30.47   & 29.36      & 30.03 & 30.09   & 29.83   & 29.27   & 29.97   & 29.36      & 29.63 & 29.58   \\
DIV2K    & 31.74   & 31.52   & 32.22   & 31.28      & 31.67 & 31.61   & 31.58   & 31.163  & 31.87   & 31.22      & 31.46 & 31.41   \\
Set12    & 30.97   & 30.78   & 31.39   & 30.40      & 30.85 & 30.88   & 30.78   & 30.40   & 31.00   & 30.31      & 30.65 & 30.59  \\ \hline\hline
\end{tabular}}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}


\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR) for noise $\sigma = 15,25,50$ on BSD68, Urban100, DIV2K, Set12, and per pixel computational cost (kFLOPs/pixel) by different methods. The symbol "-" denotes that the corresponding results are not provided.}
\label{table:compare}
\resizebox{\linewidth}{!}{
\begin{tabular}{ll|lllllllllll} \hline\hline
Dataset                   & $\sigma$                & DnCNN & CARN64  & EDSR64  & RED   & MemNet & FOCNet & SGN     & SC-CARN & SC-EDSR \\\hline
\multirow{BSD68}    &  15 & 31.97     & 32.10 & 32.16   & 32.07    & 32.14      & \textbf{32.20}  & 32.02          & 32.01   & 32.08   \\
                          & 25 & 29.58 & 29.63 & 29.70    & 29.66 & 29.67  & 29.72  & 29.65      & 29.65   & \textbf{29.76}   \\
                          & 50 & 26.54 & 26.70 & 26.84  & 26.73 & 26.74  & 27.04  & 26.77    & 27.21   & \textbf{27.31}   \\ \hline
\multirow{Urban100} & 15   & 32.85     & 32.95 & 33.10  & 32.59     & 32.50      & \textbf{33.15}  & 32.57         & 32.76   & 32.93   \\
                          & 25   & 30.04     & 30.02 & 30.36   & 29.93 & 29.91  & \textbf{30.64}  & 30.05    & 29.83 & 30.17 \\
                          & 50   & 26.30     & 26.33 & 26.85  & 26.29     & 26.34      & \textbf{27.10}  &  26.35          & 26.76   & 27.07   \\ \hline
\multirow{DIV2K}    & 15   & 33.93     & 34.04 & \textbf{34.14}   & 34.04     & 33.99      & -      & 34.02     & 33.95   & 34.03   \\
                          & 25   & 31.39 & 31.53 & 31.66  & 31.56 & 31.58  & -      & 31.68      & 31.58   & \textbf{31.75}   \\
                          & 50   & 28.25 & 28.40 & 28.65  & 28.53     & 28.43      & -      & 28.53     & 29.02   & \textbf{29.17}   \\ \hline
\multirow{Set12}    & 15   & 33.16     & 33.16 & 33.34  & 33.11     & 33.15      & \textbf{33.38}  & 33.07       & 33.14   & 33.18   \\
                          & 25   & 30.73     & 30.76 & 30.95  & 30.96 & 30.78  & 30.73  & 30.81      & 30.78   & \textbf{30.97}   \\
                          & 50   & 27.44     & 27.58 & 27.86  & 27.50 & 27.48  & 27.99  & 27.62       & 28.16   & \textbf{28.33}  \\ \hline
\multicolumn{2}{c|}{kFLOPs/pixel}        & 1108.2 & 702.7  & 2361.6  & 1106.4   & 5480.0 & 2225.7 & 429.1   & 75.5 & 148.0 \\ \hline \hline
\end{tabular}}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

%%%% original shitty ablation table
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR) with noise $\sigma = 25$ by different class settings.}
\label{table:ablationclass}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll|llllll} \hline \hline
& \multicolumn{6}{c|}{EDSR}  & \multicolumn{6}{c}{CARN} \\
Dataset  & CS & 16 & GT & NOISE & $\phi_4$ & CE & CS & 16 & GT & NOISE & $\phi_4$ & CE \\ \hline
BSD68    & 29.76   & 29.60   & 30.224  & 29.42      & 29.69 & 29.69   & 29.65   & 29.36   & 29.9    & 29.36      & 29.62 & 29.51   \\
Urban100 & 30.17   & 29.96   & 30.47   & 29.36      & 30.03 & 30.09   & 29.83   & 29.27   & 29.97   & 29.36      & 29.63 & 29.58   \\
DIV2K    & 31.74   & 31.52   & 32.22   & 31.28      & 31.67 & 31.61   & 31.58   & 31.16  & 31.87   & 31.22      & 31.46 & 31.41   \\
Set12    & 30.97   & 30.78   & 31.39   & 30.40      & 30.85 & 30.88   & 30.78   & 30.40   & 31.00   & 30.31      & 30.65 & 30.59  \\ \hline\hline
\end{tabular}}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}


\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR) with noise $\sigma = 25$ by differentd depths and widths. $N_B12$ and $N_B8$ denotes using 12 and 8 CSRB or residual blocks in the EDSR architecture. $C_f32$ and $C_f8$ denotes setting the number of feature channels to 32 or 8 for EDSR or CARN architecture. CS denotes integrating CSConv layers into the network as described in \ref{sec: csdn}.}
\label{table:ablationwidth}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|lllllllll|lllll} \hline\hline
 & \multicolumn{9}{c|}{EDSR} & \multicolumn{5}{c}{CARN}\\
Dataset  & CS    & CS,$N_B12$ & $N_B12$   & CS,$N_B8$ & $N_B8$    & CS,$C_f32$ & $C_f32$   & CS, $C_f8$ & $C_f8$    & CS    & CS,$C_f32$ & $C_f32$   & CS,$C_f8$ & $C_f8$    \\ \hline
BSD68    & 29.76 & 29.67  & 29.48 & 29.61 & 29.36 & 29.79  & 29.66 & 29.55 & 29.37 & 29.65 & 29.62  & 29.41 & 29.27 & 28.86 \\
Urban100 & 30.17 & 29.82  & 29.59 & 29.78 & 29.28 & 30.23  & 30.07 & 29.60 & 28.87 & 29.83 & 29.84  & 29.53 & 29.08 & 28.06 \\
DIV2K    & 31.74 & 31.64  & 31.36 & 31.58 & 31.20 & 31.83  & 31.62 & 31.51 & 31.22 & 31.58 & 31.59  & 31.31 & 31.20 & 30.65 \\
Set12    & 30.97 & 30.81  & 30.56 & 30.74 & 30.39 & 30.99  & 30.86 & 30.64 & 30.14 & 30.78 & 30.80  & 30.43 & 30.29 & 29.62 \\ \hline\hline
\end{tabular}}
\end{center}
\end{table}



\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR/SSIM) by EDSR models with feature channels $C_f = 16$ and different number of blocks.}
\label{table:ablationclass}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll} \hline \hline
%Dataset  & CS & 16 & G & N & $\phi_4$ & CE & CS & 16 & G & N & $\phi_4$ & CE \\ \hline
$N_B$    & 16 & 16  & 12   & 12  & 8 & 8   \\
CSConv    & Y & N   & Y   & N  & Y & N   \\ \hline
BSD68    & 29.76   & 29.60   & 29.67  & 29.48 & 29.61 & 29.36     \\
Urban100 & 30.17   & 29.96   & 29.82  & 29.59 & 29.78 & 29.28     \\
DIV2K    & 31.74   & 31.52   & 31.64  & 31.36 & 31.58 & 31.20    \\
Set12    & 30.97   & 30.78   & 30.81  & 30.56 & 30.74 & 30.39    \\ \hline\hline
\end{tabular}}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR/SSIM) by EDSR models with number of blocks $N_B = 16$ and different number of feature channels.}
\label{table:ablationclass}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll} \hline \hline
%Dataset  & CS & 16 & G & N & $\phi_4$ & CE & CS & 16 & G & N & $\phi_4$ & CE \\ \hline
$C_f$    & 32 & 32  & 16   & 16  & 8 & 8   \\
CSConv    & Y & N   & Y   & N  & Y & N   \\ \hline
BSD68  & 29.79  & 29.66 & 29.76   & 29.60  & 29.55 & 29.37      \\
Urban100 & 30.23  & 30.07 & 30.17   & 29.96  & 29.60 & 28.87      \\
DIV2K   & 31.83  & 31.62 & 31.74   & 31.52   & 31.51 & 31.22   \\
Set12   & 30.99  & 30.86 & 30.97   & 30.78  & 30.64 & 30.14    \\ \hline\hline
\end{tabular}}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR/SSIM) by CARN models with different number of feature channels.}
\label{table:ablationclass}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll} \hline \hline
%Dataset  & CS & 16 & G & N & $\phi_4$ & CE & CS & 16 & G & N & $\phi_4$ & CE \\ \hline
$C_f$    & 32 & 32  & 16   & 16  & 8 & 8   \\
CSConv    & Y & N   & Y   & N  & Y & N   \\ \hline
BSD68  & 29.62  & 29.41  & 29.65   & 29.36  & 29.27 & 28.86      \\
Urban100 & 29.84  & 29.53 & 29.83   & 29.27  & 29.08 & 28.06      \\
DIV2K   & 31.59  & 31.31  & 31.58   & 31.16 & 31.20 & 30.65   \\
Set12    & 30.80  & 30.43 & 30.78   & 30.40  & 30.29 & 29.62    \\ \hline\hline
\end{tabular}}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
%


\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Denoising performance (PSNR) with noise $\sigma = 25$ by different class settings. CS denotes the proposed model where pixel-wise classes are predicted by PCN, and $M_{\phi} = 8$, $M_{\lambda} = M_{\mu} = 3$. 16 denotes the baseline models without using CSConv, where the number of feature channels $C_f = 16$ is the same as CS. GT and NOISE use classes produced by RAISR classification on noise-free and noisy images respectively, and the number of classes is the same as CS. $\phi_4$ and $\lambda_2\mu_2$ use classes predicted by PCN, while the class number of $\phi_4$ is reduced to $M_{\phi} = 4$, $M_{\lambda} = M_{\mu} = 3$, and the class number of $\lambda_2\mu_2$ is reduced to $M_{\phi} = 8$, $M_{\lambda} = M_{\mu} = 2$.}
\label{table:ablationclass}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll|llllll} \hline \hline
& \multicolumn{6}{c|}{EDSR}  & \multicolumn{6}{c}{CARN} \\
Dataset  & CS & 16 & GT & NOISE & $\phi_4$ & $\lambda_2\mu_2$  & CS & 16 & GT & NOISE & $\phi_4$ & $\lambda_2\mu_2$  \\ \hline
BSD68    & 29.76   & 29.60/0.822   & 30.224/0.847  & 29.42/0.814      & 29.69/0.824 & 29.71   & 29.65   & 29.36   & 29.9    & 29.36      & 29.62 & 29.57   \\
Urban100 & 30.17   & 29.96/0.878   & 30.47/0.896   & 29.36/0.866      & 30.03/0.880 & 30.09   & 29.83   & 29.27   & 29.97   & 29.36      & 29.63 & 29.69   \\
DIV2K    & 31.74   & 31.52/0.856   & 32.22/0.878   & 31.28/0.849      & 31.67/0.859 & 31.69   & 31.58   & 31.16  & 31.87   & 31.22      & 31.46 & 31.50   \\
Set12    & 30.97   & 30.78/0.849   & 31.39/0.868   & 30.40/0.840      & 30.85/0.851 & 30.90   & 30.78   & 30.40   & 31.00   & 30.31      & 30.65 & 30.68  \\ \hline\hline
\end{tabular}}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}








\begin{figure*}[!t]\footnotesize
	\begin{center}
	    \begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/79073_x1_HR.png} 
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/GT79073_result_0.png} 
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/GT79073_result_1.png}
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/GT79073_result_2.png}
		\end{tabular}
		\\
%
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/79073_x1_LR.png} 
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/NOISE79073_result_0.png} 
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/NOISE79073_result_1.png}
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/NOISE79073_result_2.png}
		\end{tabular}\\
%
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/79073_x1_SR_carn.png} 
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/SR79073_result_0.png} 
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/SR79073_result_1.png}
		\end{tabular}
		\begin{tabular}{c}
			\includegraphics[width=\swfour]{\figdir/SR79073_result_2.png}
		\end{tabular}
	\end{center}
	\vspace{-3mm}
	\caption{
		Visualization of gradient statistics obtained from noise-free image ($1^{st}$ row), noisy image ($2^{nd}$ row) according to the eigen analysis in RAISR~\cite{romano2016raisr} as well as the proposed PCN prediction from noisy image ($3^{rd}$ row).
		%
		The four columns represent grayscale image, $\phi$, $\lambda$, and $\mu$ respectively.
		%
		It shows that the estimation accuracy is limited by the eigen analysis when the input is contaminated by noises.
		%
		The proposed PCN can predict more accurate gradient statistics after training with those obtained from noise-free image by the eigen analysis and more accurate gradient statistics will lead to better pixel-wise classification.
	}
	\label{fig:classes}
\end{figure*}


\begin{figure*}[!t]
	\begin{center}
		\begin{tabular}{cccccccccc}
			\includegraphics[width=\swten]{figs4/0041_x1_HR.png}&
			\includegraphics[width=\swten]{figs4/0041_x1_HR_crop.png}&
			\includegraphics[width=\swten]{figs4/0041_x1_LR.png} &
			\includegraphics[width=\swten]{figs4/0041_x1_LR_crop.png} &
			\includegraphics[width=\swten]{figs4/0041_x1_SR_gt.png}&
			\includegraphics[width=\swten]{figs4/0041_x1_SR_gt_crop.png}&
			\includegraphics[width=\swten]{figs4/0041_x1_SR_noise.png}&
			\includegraphics[width=\swten]{figs4/0041_x1_SR_noise_crop.png} &
			\includegraphics[width=\swten]{figs4/0041_x1_SR_csedsr.png}&
			\includegraphics[width=\swten]{figs4/0041_x1_SR_csedsr_crop.png} \\		
			\multicolumn{2}{c}{(a) clean } & \multicolumn{2}{c}{(b) noisy }  & \multicolumn{2}{c}{(d) RAISR+C }& \multicolumn{2}{c}{ (e) RAISR+N }  & \multicolumn{2}{c}{(c) PCN+N } \\
			\multicolumn{2}{c}{PSNR/SSIM } & \multicolumn{2}{c}{ 20.56/0.362 }  & \multicolumn{2}{c}{ 30.33/0.836 }& \multicolumn{2}{c}{ 29.42/0.780 }  & \multicolumn{2}{c}{ 29.80/0.798 } \\
			\end{tabular}
			\begin{tabular}{ccccccccc}
			\includegraphics[width=\swnine]{figs4/GT0041_result_0_cropped1.png} &
			\includegraphics[width=\swnine]{figs4/GT0041_result_1_cropped1.png} &
			\includegraphics[width=\swnine]{figs4/GT0041_result_2_cropped1.png} &
			\includegraphics[width=\swnine]{figs4/NOISE0041_result_0_cropped1.png} &
			\includegraphics[width=\swnine]{figs4/NOISE0041_result_1_cropped1.png} &
			\includegraphics[width=\swnine]{figs4/NOISE0041_result_2_cropped1.png} &
			\includegraphics[width=\swnine]{figs4/SR0041_result_0_cropped1.png} &
			\includegraphics[width=\swnine]{figs4/SR0041_result_1_cropped1.png} &
			\includegraphics[width=\swnine]{figs4/SR0041_result_2_cropped1.png} \\
		\multicolumn{3}{c}{(f) RAISR+C } & \multicolumn{3}{c}{(g) RAISR+N }  & \multicolumn{3}{c}{(h) PCN+N }\\
		\multicolumn{3}{c}{MSE } & \multicolumn{3}{c}{ 0.063 }  & \multicolumn{3}{c}{ 0.029 }\\
		
		\end{tabular}
	\end{center}
	\vspace{-3mm}
	\caption{
		Top row: visual comparison by different classification methods on BSD68 \cite{martin2001database} with $\sigma =25$ noise. As can be seen in the zoomed area, PCN+N and RAISR+C recover the sharpness and the direction of the stripe pattern. Bottom row: visualized comparison of gradient statistics produced by different classification methods. For each method, three figures from left to right denote the pixel-wise gradient statistics $\phi$, $\lambda$ and $\mu$. PCN produces a close estimate of the RAISR+C while RAISR+N is disrupted by the existence of noises.
		%
	}
	\label{fig:effective}
\end{figure*}


\begin{figure*}[!t]
	\begin{center}
		\begin{tabular}{cccccc}
			\includegraphics[width=\swsix]{figs3/barbara_x1_HR.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_LR.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB16C16.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B16C16.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB16C32.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B16C32.png} \\
			\includegraphics[width=\swsix]{figs3/barbara_x1_HR_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_LR_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB16C16_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B16C16_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB16C32_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B16C32_crop.png} \\
			(a) clean & (b) noisy & (c) CS-B16C16 & (d) B16C16 & (e) CS-B16C32 & (f) B16C32 \\
			PSNR/SSIM & 20.42/0.395 & 30.21/0.877 & 30.01/0.871 & 30.29/0.879 & 30.23/0.878  \\
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB8C16.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B8C16.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB12C16.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B12C16.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB16C8.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B16C8.png} \\
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB8C16_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B8C16_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB12C16_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B12C16_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_csB16C8_crop.png} &
			\includegraphics[width=\swsix]{figs3/barbara_x1_SR_B16C8_crop.png} \\
			(g) CS-B8C16 & (h) B8C16 & (i) CS-B12C16 & (j) B12C16 & (k) CS-B16C8 & (l) B16C8 \\
			29.82/0.867 & 29.28/0.849 & 29.85/0.868 & 29.45/0.860 & 29.58/0.861 & 28.83/0.839 \\
		\end{tabular}
	\end{center}
	\vspace{-3mm}
	\caption{
		Visual comparison by CS-EDSR and EDSR with different number of blocks and features on Set12~\cite{zhang2017beyond} with $\sigma =25$ noise.
		%
		Model names with and without CS- denote CS-EDSR and EDSR, respectively.
		%
		BiCj denotes the number of blocks and feature channels as i and j, respectively. 
		%
		As can be seen in the zoomed areas, when using fewer blocks or features, CS-EDSR still produces relatively clear details, whereas the results of EDSR are smoother.
	}
	\label{fig:ablationblocks}
\end{figure*}

